A reduction theorem for L\^e's conjecture

Let $\boldsymbol{n}=(n_1,n_2,n_3):(\mathbb{C}^2,0)\to(\mathbb{C}^3,0)$ be a holomorphic map germ admitting an injective representative. We prove that if $(d\boldsymbol{n})_0=0$, then $\mathrm{ord}_0(\boldsymbol{n})\in\{2,3,4\}$. This reduces L\^e's conjecture to excluding potential counterexamples $\boldsymbol{n}$ of orders $2$, $3$, and $4$. The proof combines techniques from the theory of plane curve singularities, explicit cobordism constructions, and genus bounds obtained by applying properties of the $\Upsilon$ invariant coming from knot Floer homology.

==> plane_sections_draft_labels.tex <==
%% Creator: Inkscape 1.4.4 (dcaf3e7d9e, 2026-05-05), www.inkscape.org
%% PDF/EPS/PS + LaTeX output extension by Johan Engelen, 2010
%% Accompanies image file 'plane_sections_draft.pdf' (pdf, eps, ps)
%%
%% To include the image in your LaTeX document, write
%%   \input{<filename>.pdf_tex}
%%  instead of
%%   \includegraphics{<filename>.pdf}
%% To scale the image, write
%%   \def\svgwidth{<desired width>}
%%   \input{<filename>.pdf_tex}
%%  instead of
%%   \includegraphics[width=<desired width>]{<filename>.pdf}
%%
%% Images with a different path to the parent latex file can
%% be accessed with the `import' package (which may need to be
%% installed) using
%%   \usepackage{import}
%% in the preamble, and then including the image with
%%   \import{<path to file>}{<filename>.pdf_tex}
%% Alternatively, one can specify
%%   \graphicspath{{<path to file>/}}
%% 
%% For more information, please see info/svg-inkscape on CTAN:
%%   http://tug.ctan.org/tex-archive/info/svg-inkscape
%%
\begingroup%
  \makeatletter%
  \providecommand\color[2][]{%
    \errmessage{(Inkscape) Color is used for the text in Inkscape, but the package 'color.sty' is not loaded}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\transparent[1]{%
    \errmessage{(Inkscape) Transparency is used (non-zero) for the text in Inkscape, but the package 'transparent.sty' is not loaded}%
    \renewcommand\transparent[1]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \newcommand*\fsize{\dimexpr\f@size pt\relax}%
  \newcommand*\lineheight[1]{\fontsize{\fsize}{#1\fsize}\selectfont}%
  \ifx\svgwidth\undefined%
    \setlength{\unitlength}{459.21259843bp}%
    \ifx\svgscale\undefined%
      \relax%
    \else%
      \setlength{\unitlength}{\unitlength * \real{\svgscale}}%
    \fi%
  \else%
    \setlength{\unitlength}{\svgwidth}%
  \fi%
  \global\let\svgwidth\undefined%
  \global\let\svgscale\undefined%
  \makeatother%
  \begin{picture}(1,0.5859375)%
    \lineheight{1}%
    \setlength\tabcolsep{0pt}%
    \put(0,0){\includegraphics[width=\unitlength,page=1]{plane_sections_draft.pdf}}%
    \put(0.19140625,0.5296875){\color[rgb]{0.1254902,0.14901961,0.17254902}\makebox(0,0)[t]{\lineheight{1.25}\smash{\begin{tabular}[t]{c}$\mathbb C^2$\end{tabular}}}}%
    \put(0.75468751,0.5296875){\color[rgb]{0.1254902,0.14901961,0.17254902}\makebox(0,0)[t]{\lineheight{1.25}\smash{\begin{tabular}[t]{c}$X\subset\mathbb C^3$\end{tabular}}}}%
    \put(0.4546875,0.53984375){\color[rgb]{0.1254902,0.14901961,0.17254902}\makebox(0,0)[t]{\lineheight{1.25}\smash{\begin{tabular}[t]{c}$\boldsymbol n$\end{tabular}}}}%
    \put(0.17265625,0.2734375){\color[rgb]{0.1254902,0.14901961,0.17254902}\makebox(0,0)[lt]{\lineheight{1.25}\smash{\begin{tabular}[t]{l}$0$\end{tabular}}}}%
    \put(0.13828125,0.10390625){\color[rgb]{0,0.55686275,0.60784314}\makebox(0,0)[t]{\lineheight{1.25}\smash{\begin{tabular}[t]{c}$V=V_0$\end{tabular}}}}%
    \put(0.2640625,0.10390625){\color[rgb]{0,0.55686275,0.60784314}\makebox(0,0)[t]{\lineheight{1.25}\smash{\begin{tabular}[t]{c}$V_s$\end{tabular}}}}%
    \put(0.1359375,0.0453125){\color[rgb]{0.1254902,0.14901961,0.17254902}\makebox(0,0)[t]{\lineheight{1.25}\smash{\begin{tabular}[t]{c}$V_0=\{v=0\}$\end{tabular}}}}%
    \put(0.31171875,0.0453125){\color[rgb]{0.1254902,0.14901961,0.17254902}\makebox(0,0)[t]{\lineheight{1.25}\smash{\begin{tabular}[t]{c}$V_s=\{v=s\}$\end{tabular}}}}%
    \put(0.22109375,0.01171875){\color[rgb]{0.1254902,0.14901961,0.17254902}\makebox(0,0)[t]{\lineheight{1.25}\smash{\begin{tabular}[t]{c}$v=\lambda_1\circ\boldsymbol n$\end{tabular}}}}%
    \put(0.36171875,0.32734375){\color[rgb]{0.1254902,0.14901961,0.17254902}\makebox(0,0)[t]{\lineheight{1.25}\smash{\begin{tabular}[t]{c}$V_0$\end{tabular}}}}%
    \put(0.55,0.32734375){\color[rgb]{0.1254902,0.14901961,0.17254902}\makebox(0,0)[t]{\lineheight{1.25}\smash{\begin{tabular}[t]{c}$W_0$\end{tabular}}}}%
    \put(0.45546875,0.34296875){\color[rgb]{0.1254902,0.14901961,0.17254902}\makebox(0,0)[t]{\lineheight{1.25}\smash{\begin{tabular}[t]{c}$\boldsymbol n_0$\end{tabular}}}}%
    \put(0.36171875,0.21171875){\color[rgb]{0.1254902,0.14901961,0.17254902}\makebox(0,0)[t]{\lineheight{1.25}\smash{\begin{tabular}[t]{c}$V_s$\end{tabular}}}}%
    \put(0.55,0.21171875){\color[rgb]{0.1254902,0.14901961,0.17254902}\makebox(0,0)[t]{\lineheight{1.25}\smash{\begin{tabular}[t]{c}$W_s$\end{tabular}}}}%
    \put(0.45546875,0.22734375){\color[rgb]{0.1254902,0.14901961,0.17254902}\makebox(0,0)[t]{\lineheight{1.25}\smash{\begin{tabular}[t]{c}$\boldsymbol n_s$\end{tabular}}}}%
    \put(0.65000001,0.48515625){\color[rgb]{0.1254902,0.14901961,0.17254902}\makebox(0,0)[t]{\lineheight{1.25}\smash{\begin{tabular}[t]{c}$H_0=\{\lambda_1=0\}$\end{tabular}}}}%
    \put(0.82890626,0.48515625){\color[rgb]{0.1254902,0.14901961,0.17254902}\makebox(0,0)[t]{\lineheight{1.25}\smash{\begin{tabular}[t]{c}$H_s=\{\lambda_1=s\}$\end{tabular}}}}%
    \put(0.6640625,0.2640625){\color[rgb]{0.1254902,0.14901961,0.17254902}\makebox(0,0)[lt]{\lineheight{1.25}\smash{\begin{tabular}[t]{l}$0$\end{tabular}}}}%
    \put(0.646875,0.0453125){\color[rgb]{0,0.55686275,0.60784314}\makebox(0,0)[t]{\lineheight{1.25}\smash{\begin{tabular}[t]{c}$W=W_0=X\cap H_0$\end{tabular}}}}%
    \put(0.8046875,0.2734375){\color[rgb]{0,0.55686275,0.60784314}\makebox(0,0)[t]{\lineheight{1.25}\smash{\begin{tabular}[t]{c}$W_s$\end{tabular}}}}%
    \put(0.85312501,0.01171875){\color[rgb]{0,0.55686275,0.60784314}\makebox(0,0)[t]{\lineheight{1.25}\smash{\begin{tabular}[t]{c}$W_s=X\cap H_s$\end{tabular}}}}%
    \put(0.84375,0.434375){\color[rgb]{0.4745098,0.32156863,0.63921569}\makebox(0,0)[t]{\lineheight{1.25}\smash{\begin{tabular}[t]{c}$\Sigma_1$\end{tabular}}}}%
    \put(0.84375,0.11328125){\color[rgb]{0.4745098,0.32156863,0.63921569}\makebox(0,0)[t]{\lineheight{1.25}\smash{\begin{tabular}[t]{c}$\Sigma_2$\end{tabular}}}}%
    \put(0.778125,0.38828125){\color[rgb]{0.1254902,0.14901961,0.17254902}\makebox(0,0)[rt]{\lineheight{1.25}\smash{\begin{tabular}[t]{r}{\scalebox{0.65}{\scriptsize $Q_1(s)$}}\end{tabular}}}}%
    \put(0.778125,0.3375){\color[rgb]{0.1254902,0.14901961,0.17254902}\makebox(0,0)[rt]{\lineheight{1.25}\smash{\begin{tabular}[t]{r}{\scalebox{0.65}{\scriptsize $Q_2(s)$}}\end{tabular}}}}%
    \put(0.778125,0.2109375){\color[rgb]{0.1254902,0.14901961,0.17254902}\makebox(0,0)[rt]{\lineheight{1.25}\smash{\begin{tabular}[t]{r}{\scalebox{0.65}{\scriptsize $Q_3(s)$}}\end{tabular}}}}%
    \put(0.778125,0.16328125){\color[rgb]{0.1254902,0.14901961,0.17254902}\makebox(0,0)[rt]{\lineheight{1.25}\smash{\begin{tabular}[t]{r}{\scalebox{0.65}{\scriptsize $Q_4(s)$}}\end{tabular}}}}%
  \end{picture}%
\endgroup%

